FireGuard: A Generalized Microarchitecture for Fine-Grained Security Analysis on OoO Superscalar Cores

High-performance security guarantees rely on hardware support. Generic programmable support for fine-grained instruction analysis has gained broad interest in the literature as a fundamental building block for the security of future processors. Yet, implementation in real out-of-order (OoO) superscalar processors presents tough challenges that cannot be explored in highly abstract simulators. We detail the challenges of implementing complex programmable pathways without critical paths or contention. We then introduce FireGuard, the first implementation of fine-grained instruction analysis on a real OoO superscalar processor. We establish an end-to-end system, including microarchitecture, SoC, ISA and programming model. Experiments show that our solution simultaneously ensures both security and performance of the system, with parallel scalability. We examine the feasibility of building FireGuard into modern SoCs: Apple's M1-Pro, Huawei's Kirin-960, and Intel's i7-12700F, where less than 1% silicon area is introduced. The Repo. of FireGuard's source code: https://github.com/SEU-ACAL/reproduce-FireGuard-DAC-25.

==> Meeting_notes.tex <==
L1 Cache (1-2 cycle latency) xxx
Risk I: L1 is not designed for sharing, but ETH paper is an evidence
Risk II: How to deal with D$ and I$

L2 Cache (4-8 cycle latency) 
-- A better choice
-- We need to compare this work with cache coloring \& partitioning 
-- Zhe Jiang will review this.
Risk I: What is the difference between cache coloring and partitioning?
-- Low-granularity
-- How to deal with cache coherence?


Processor (Suggest to do something here)
-- We have full control of the processor design, we have two options: (i) a 5-stage pipeline processor; (ii) a 10-stage pipeline superscalar processor 
-- We will use 5-stage pipeline processor 

Virtual address
-- We only focus on the threads in the same process, therefore, the addresses are shared between all DAG nodes.






READ THIS PAPER --- Real-Time Scheduling of Autonomous Driving System with Guaranteed Timing Correctness (for story line)

Relationship between node WCET \& cache size
--- could cite this: llvm Timing Analysis


==> abstract_old.tex <==
\begin{abstract}
Systems and software security is becoming increasingly challenging due to the presence of untrusted and ever-more complex applications. 
Conventional analyzers typically involve trade-offs in overhead and flexibility, making it challenging to provide robust, updateable security protection.

The Guardian Council is a heterogeneous and parallel architecture for comprehensive analysis. 
Through processor observation channels and heterogeneous parallelism via a sea of microcontroller-sized programmable checker cores ($\mu$cores), it can support various security validations with low overhead and offers flexibility for customization. 
However, building a real system like this is challenging due to an absence of microarchitectural details.

Here we present the first microarchitecture for the Guardian Council: \marchname{}. 
To achieve comprehensive and efficient monitoring of the compute core, we introduce: a buffer-free data-forwarding channel that extracts the execution data of the compute core with light microarchitectural changes and without adding holding space for speculative intermediates inside the core;
an SRAM-based superscalar event filter that pre-checks all instruction commits in parallel, without impeding system-wide performance; and a broadcast-free mapper that enables timely data movement across the compute core and $\mu$cores.
To optimize the execution of online security validations, we extend RISC-V's custom-instruction interface to tightly integrate it into the pipeline of $\mu$cores, accompanied by corresponding programming models, which ensures low-latency hardware-software interactions. 
% \sam{Hugo is this RISC-V's custom-instruction interface or RISC-V Rocket's? Anyway I altered it to say more about what we did, otherwise it reads more like we did ``jargon jargon jargon jargon that I, the reviewer, can skip''}
% \hugo{Sam, I am with you. More precisely, it is a UCB's RISC-V's ISAX interface used in both Rocket and BOOM. However, I noticed that most of the ISAX interfaces have very similar designs (although the RISC-V specification does not regulate this), and the reviewers will not be clear about that. I have changed some [Rocket RISC-V ISAX interfaces] to [RISC-V Interfaces] in the paper (not all of them). What do you think about them, and do you have any other suggestions about this?} \sam{Yep fine, go with that.}

We build \marchname{} based on an out-of-order superscalar RISC-V BOOM core using real RTL and deploy the design on Virtex UltraScale+ FPGAs using FireSim. 
The experimental results examine FireGuard using comprehensive metrics. 
For instance, four $\mu$cores are sufficient to deploy a custom performance counter at only 2.5\% performance overhead, a shadow stack at 2.1\% overhead, or an AddressSanitizer-like scheme at 39\% overhead, dropping to 6\% with 12 $\mu$cores.
Integrating hardware accelerators into \marchname 's filtering-mapping mechanisms removes performance overhead almost completely.
We further explore the feasibility of building \marchname\ in modern SoCs: Apple's M1-Pro, Huawei's Kirin-960, and Intel's i7-12700F, where less than 1\% silicon area is introduced.
\end{abstract}
 

==> checker.tex <==

\begin{figure*}[t]
    \centering
    %No vspace before figures -- goes out of margins
    \includegraphics[width=1\linewidth]{graphics/ISAX.pdf}
    \vspace{-20pt}
    \caption{Custom instructions are integrated into the $\mu$core's pipeline at the MA stage. \textit{(gray lines: control paths; MSQ\_Ctrl: Message Queue Controller;
    IFU: Instruction Fetch Unit; Mini-D: Mini-Decoder):}
    For the ISAX interface (IFC), a full-duplex microarchitecture handles requests and responses independently, with a mini-decoder and multiplexer. 
    In the request channel, a mini-decoder directs an ISAX request to the message queues' MSQ\_Ctrl or status registers (via an APB bridge).
    In the response channel, a multiplexer selects returned data, routing it to the commit stage and the EX stage using forwarding logic for handling data hazards. }
    \vspace{-8pt}
    \label{fig:ISAX}
\end{figure*}

\vspace{-10pt}
\subsection{ISA and Programming Model}
\label{sc:Security chckers}
The analysis engines run guardian kernels concurrently on $\mu$cores, finding vulnerabilities. 
To handle the frequent hardware-software interactions, we use a FIFO-based programming model implemented into RISC-V Rocket cores via custom instructions. 
As these instructions take up a large fraction of total $\mu$core cycles, we integrate FIFO-management instructions using a new tight-coupling arrangement; Rocket's existing ISAX interface, which executes custom instructions post-commit, caused too many data hazards. 
We also redesign our instruction set to better support high-throughput programming design patterns that minimize hazards further.
%This full-stack methodology allows our $\mu$cores to process data at high efficiency, spending clock cycles on real computation instead of data management.

%we design a pipeline-coupled ISAX interface and seamlessly integrated it into the $\mu$core's pipeline.
%This design achieves low-latency hardware-software interactions and guarantees such interactions incur only a light timing penalty for the $\mu$cores' pipeline execution.
%\sam{There are a lot of meaningless words in the above. ``low latency'' ``seamlessly'', and ``a pipeline-coupled ISAX interface'' sounds like you just added a custom instruction, which the reviewer will think is boring. WHICH COULD NOT BE FURTHER FROM THE TRUTH. What is the single most important thing you want the reader to get from this? I think it's the non-standard coupling point of the ISAX instruction. Because you need to use these custom instructions very frequently, they need to be before the post-commit stages in the default Rocket design. Because it is non-speculative, it has to be after execute. Bring out the non-standardness of your design, and how well principled it was, right here. IE bring out the most interesting part of your design choices, or your reviewer will just skip this section and think it's bulk text. To be clear, the standard approaches offered in Rocket were not good enough for your use case, so you had to use your own ingenuity to do better to properly evaluate your microarchitecture. Don't let the reviewer miss that point. You also want to be clear that the interface is to do with FIFOs here, which isn't obvious until the next section, and doubly makes it look like this is just about you adding a custom instruction, which is not research.}

%\vspace{-5pt}
%\subsection{ISA and Microarchitecture}
% \label{sbsc:ISAX:Microarchitecture}
% \vspace{-3pt}



% The analysis engines interface with the main core via filtered and mapped instruction copies. 
% These are accessed by the $\mu$cores via custom instructions and the interfaces of the message queues. 
% However, we had to extend the standard RISC-V ISAX interface, bringing it further inside the core, to make it perform well.

\parlabel{ISA.} 
We connect the message queues to the fabric network in the mapper, allowing the $\mu$core to receive packets via an input queue and send packets through an output queue, in order to support pipelined parallelism strategies such as used in the shadow stack~\cite{ainsworth2020guardian}.
Our queue controller, with status registers and software drivers, allows guardian kernels to manage the message queues using ISAX~\cite{asanovic2016rocket} custom instructions (see table~\ref{table:ISA}). \texttt{Top}, \texttt{push} and \texttt{pop} were inherited from the original design~\cite{ainsworth2020guardian}; \texttt{count} was added to aid in loop unrolling, and \texttt{recent} to allow accessing extra information about an element already processed: for example, the PC is only needed on a detected error in AddressSanitizer, and is discarded otherwise.

%\sam{Is that right? Semi-relatedly, does that interact badly with unrolling?}.
% \hugo{Sorry, I did not get you.} \sam{I altered the text here to say what recent does -- is my description of what it does in ASAN correct? And given we unroll, which causes multiple Pops to appear next to each other, does that mean that Recent doesn't always give us the data we want, because we've already popped multiple by the time we've processed the data?}




\parlabel{Microarchitecture Support.} 
RISC-V Rocket executes custom instructions post-commit~\cite{asanovic2016rocket}.
The routing to the ISAX peripheral blocks the core for at least 3 cycles 
for each instruction and can extend up to 13 cycles in the presence of data hazards and contention~\cite{Pala2017rocc}.
This causes data hazards and large slowdowns when such instructions are as commonly used as our queue operations. We redesigned Rocket's interface to move it into the MA stage\footnote{The MA stage was chosen as it is the first stage in the pipeline that is non-speculative, simplifying the implementation of the state-destructive \texttt{pop} operation but otherwise minimizing hazards, such that only one bubble is required for an instruction immediately following the custom instruction that uses its output.} of the $\mu$core's pipeline (detailed in \cref{fig:ISAX}), multiplexing between the ISAX unit and the load-store unit.%, ensuring that an ISAX instruction can be delivered to the message queues immediately after the $\mu$core verifies its validity (\ie, a branch-prediction hit). 
%To achieve this, we employ a multiplexer and demultiplexer pair at the Memory Access (MA) pipeline stage.
%These create separate paths for different types of instructions, forwarding ISAX instructions to the ISAX interface, routing load and store instructions to the Load Store Unit (LSU), and directing other instructions directly to the Write Back (WB) pipeline stage, as shown in 

%In the ISAX interface, we introduce a full-duplex microarchitecture that independently manages ISAX requests and responses. 
%In the request channel, we deploy a mini-decoder at the entry point, directing an ISAX request to the queue controller or an AMBA APB bridge.
%The APB bridge hooks the status registers of the message queues, converting an ISAX instruction to the corresponding register index and returning the value in a fixed single clock cycle. 
%In the response channel, a multiplexer is used to select the data returned from the queue controller or the status register, then routes it back to the $\mu$core, see Fig.~\ref{fig:ISAX} (b).
%\sam{I removed the sentences about the ISAX requests/responses because it's not interesting. We now don't refer to 7b in the text though, so you may want to rejig somehow / add something into the caption.}
%\hugo{Updated: added short descriptions of the microarchitrue in Fig.7. I also changed your ref to the Figure 7, not 7(a), and added the descriptions in figure 7 for both (a) and (b).}

%\parlabel{Data hazards.}
%The proposed design may lead to data hazards in the $\mu$core's pipeline execution, \ie, the execution of an instruction may depend on the data returned from the message queues, which is requested by a previous instruction.
%To improve the efficiency of pipeline execution, we introduce data forwarding logic that routes the response data from the ISAX interface directly back to the Execution (EX) pipeline stage, as shown by the blue line in Fig.~\ref{fig:ISAX} (a). 
%This allows a dependent instruction to execute immediately with the response data, rather than waiting for the data to be stored in the general-purpose registers at the Write-back (WB) stage.

%\subsection{Design Trade-offs}
%Coupling the ISAX interface into $\mu$core's pipeline ensures low-latency hardware-software interactions, with light timing penalties of pipeline execution: a 1-cycle delay for instructions with dependencies and no delay for other instructions.

%\parlabel{Deploying ISAX interfaces to other pipeline stages.}
%To eliminate the introduced timing penalty, it is possible to integrate the ISAX interface into other pipeline stages, \eg, the Instruction Decode (ID) and EX stages. 
%However, this approach exposes the control of the message queues, where even reads are destructive, \sam{Added the previous clause} to the risk of branch prediction~\cite{hennessy2011computer}. 
%A straightforward way to address this issue is to add new functionalities to the queue controller, allowing it to revoke an executed operation. 
%Nevertheless, this addition would significantly increase hardware complexity.
%Instead, we propose a new programming model (Sec.~\ref{Sc:ProgrammingModel}) that mitigates this issue solely from the software.

%\begin{table}[t]
% \centering
%\begin{tabular}{|c|l|}                                  \hline
%u16 \textbf{count} (queue \textit{q})            & \begin{tabular}[c]{@{}l@{}}Count packets buffered in \textit{q}.\end{tabular}                \\ \hline
%u64 \textbf{recent} (bitfield \textit{b})                                                      & \begin{tabular}[c]{@{}l@{}}Return bitfields {[}\textit{b+63 : b}{]} of the\\ most recently removed element.\end{tabular} \\ \hline
%\end{tabular}
%\caption{New control instructions for message queues, in addition to the standard \textit{top}, \textit{push} and \textit{pop} from the original paper~\cite{ainsworth2020guardian}.}
%\hugo{This table looks very naive now. Shall we delete it?} \sam{By all means -- fold the text in where we mention it if it makes sense to (down at the other commented-on bit below).}
%\vspace{-16pt}
%\label{table:functions}
%\end{table}

%\vspace{-3pt}
%\subsection{Design Trade-Offs}
%\vspace{-2pt}
%Moving the ISAX interface to the MA stage, with data forwarding to EX, still leaves a load-use delay if the immediately following instruction uses the response. Implementing in EX instead would have rollback on misspeculation (and most of our common-case instructions, e.g., queue pop, are destructive). 

%Managing message queues using ISAX instructions necessitates additional compiler support. 
%To enhance compatibility and portability, an alternative approach involves encapsulating the message queues as a memory-mapped peripheral and assigning it to specific memory regions. 
%This allows control using general memory write/read operations. 
%However, memory-mapped peripherals typically incur high access delays due to extended transaction paths and additional contention~\cite{jiang2022axi,damian2022scaie,restuccia2022bounding}. 
%Hence, we adopt the pipeline-coupled interface to support communications between the $\mu$core and the message queues.
% \hugo{[To Sam]: in other sections, the design trade-offs is a dedicated subsection, but here is the parlabel. Is this intended? I am fine with either option, but better to keep the consistency?}  \sam{Yes intended, and a deliberate act of inconsistency to keep sections 7.1 amd 7.2 together (because these tradeoffs are of 7.1.}




==> design.tex <==

\section{\marchname: Microarchitecture}
\label{sc:Design}
As described in Sec.~\ref{section:Overview} and Fig.~\ref{fig:Top_Micro}, the top-level microarchitecture of \marchname\ is partitioned into four primary parts: a data-forwarding channel, an event filter, a mapper, and a group of security checkers. 
In this section, we detail the microarchitecture of each of these modules, followed by discussions on the design trade-offs and the rationales behind making the design decisions.

\subsection{Data-forwarding Channel}
\label{sbsc:Data-forwarding Channel}
The data-forwarding channel is deployed at the commit stage of the main core, extracting, selecting, and transporting debug data associated with \emph{each} retired instruction.  
Since the relevant data is already stored in different locations within the main core, we propose an \emph{implicit} microarchitecture for the data-forwarding channel by inserting bypass circuits at the Reorder Buffer (ROB), Physical Register Files (PRFs), Load Store Queue (LSQ), and Fetch Target Queue (FTQ) to transport PC address, instruction data, operand data, memory access address, and jump address for the in instruction commitment, without requiring additional buffering.
The design enables fine-grained visibility into program execution, allowing different instructions (e.g., loads, stores, jumps) and system calls to be forwarded for in-depth analysis.


\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{graphics/Data_ForwardingChannel.pdf}
    \caption{Microarchitecture of data-forwarding channel, using PRFs as an example. 
    Similar microarchitecture is respectively deployed in the LSQ and FTQ (Ctrl: Controller; DP\_Sel: Data Path Selection).
    }
    \label{fig:Data_ForwardingChannel}
\end{figure}



\parlabel{Microarchitecture.}
Fig.~\ref{fig:Data_ForwardingChannel} illustrates the microarchitecture of the data-forwarding channel using PRFs as an example, physically connecting the ROB, event filter, and PRFs.

On the ROB side, we present a combinational logic to hook on each commit width, transmitting the retired instructions to the mini-filters, as well as a group of temporary address registers, buffering the PRF addresses accessed by these instructions (Fig.~\ref{fig:Data_ForwardingChannel} (a)).
With the transmitted instructions, the mini-filters identify their G$\_$IDs and select the debug data for later analysis.
If the PRF data is selected, a control signal is routed back to the PRF controller (Fig.~\ref{fig:Data_ForwardingChannel} (b)).

On the PRF side, we introduce a set of 2-to-1 multiplexers between Issue Queues (IQs) and their statically mapped PRF read controllers~\cite{zhao2020sonicboom} (Fig.~\ref{fig:Data_ForwardingChannel} (c)).
For each multiplexer, we connect the temporary address register and a IQ's request port to the input data ports, then connect the control signal routed from the corresponding mini-filter to the control port, ensuring the desired PRF data can be read and transported preferentially after the instruction filtering (see Fig.\ref{fig:Data_ForwardingChannel} (d)).



\parlabel{Design trade-offs.}
Designing the data-forwarding channel using bypass circuits effectively minimizes modifications to the main core.
However, to ensure the correctness of the obtained data and prevent data overwriting, the data-forwarding channel must seize control of the PRF read controller immediately after instruction filtering by manipulating the corresponding multiplexer (blue box in Fig.~\ref{fig:Data_ForwardingChannel}).
Such preemption might delay the read operation issued by the IQ, resulting in an extra cycle delay for the instruction dispatch.

To eliminate this issue, an alternative approach involves introducing dedicated PRF read controllers and supplementary PRF ports solely for data forwarding. However, this microarchitecture is resource-inefficient, as adding the PRF ports can be costly, leading to a significant increase in combinational logic, which may, in turn, introduce critical paths. In \textcolor{blue}{Sec.~\ref{}}, we present a quantitative performance evaluation to assess the necessity of adding dedicated read controllers and ports, helping determine the most effective design method for balancing resource efficiency and performance in the context of data forwarding and pipeline execution.


\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{graphics/mini_Filter.pdf}
    \caption{Microarchitecture of Mini-Filter (LB: Load Byte; SB: Store Byte; WR IFC: Write Interface; RD: Read Interface).}
    \label{fig:Mini_Filter}
\end{figure}

% The event filter pre-checks all committed instructions and returns their G\_IDs.
% In coping with parallel instruction commitments, we develop a \emph{superscalar} microarchitecture for the event filter using a set of mini-filters, FIFO queues, and an arbiter, illustrated in Fig.~\ref{fig:Top_Micro}.(b).
% Each mini-filter is connected to a commit width of the main core and uses an SRAM look-up-table to capture the information used by filtering, \eg, opcode, function code, and $G\_IDs$ of the sensitive instructions.
% The filtered results are buffered in the paired FIFO queues, allowing the arbiter reorganises them using the commit order.

\subsection{Event Filter}
\label{sbsc:Event Filter}
In coping with parallel instruction commitments from the main core, we propose a \emph{superscalar} microarchitecture for the event filter that enables simultaneous filtering of the committed instructions. 
This design ensures that the event filter attains the same instruction-level parallelism as the main core, thereby preventing filtering activities from impeding system-wide performance.

\parlabel{Microarchitecture.} 
Fig.~\ref{fig:Top_Micro} (b) illustrates the microarchitecture of the event filter, including a set of mini-filters, FIFO queues, and an arbiter.
The mini-filters are connected to each commit width of the ROB to identify the G\_IDs and select the debug data for the retired instructions.
The filtered contents are temporarily stored in the paired FIFO queues, allowing the arbiter reorganises them using the commit order.


We design the mini-filter based on a configurable SRAM-based look-up table, named filter table (see Figure~\ref{fig:Mini_Filter}). 
The memory address (10-bit) is employed to index both opcode (upper 7 bits) and function code (lower 3 bits) for all possible instructions, while the memory data is utilized to store the G$\_$ID and the desired data path for each instruction.~\footnote{Note, a G$\_$ID value of `0' indicates a non-sensitive instruction.}
For instance, the addresses 0x03 and 0x23 are designated for indexing $LB$ and $SB$, respectively.
To facilitate instruction filtering, we route the committed instructions' opcode and function code to the address port of the SRAM's read interface. 
Subsequently, we direct the read data to the data-forwarding channels and the mappers, assisting data selection and allocation, respectively.
To support customisation, we map the filter table to a dedicated memory region and provide the corresponding software drivers, allowing the main core to write the table though its write interface.


\begin{figure}[h]
    \centering
    \includegraphics[width=1\columnwidth]{graphics/Re-ordering.pdf}
    \caption{Packets reordering, using the 4-width FIFO queues as an example. P[$x$].$y$: the $y$th packet in FIFO[$x$].}
    \label{fig:Re-ordering}
\end{figure}

We place a pair of FIFO queues to connect the mini-filters, which buffer the filtered contents (Fig.~\ref{fig:Re-ordering} (a)).
Although these filtered contents are produced by the mini-filters in parallel, they must be sent sequentially, aligning with their commit order. 
This is crucial because guardian kernels (\eg, ShadowStack~\cite{}) might be sensitive to the order of instruction commitments.
With this in mind, we develop an encapsulation format to pack the filtered contents, see Fig.~\ref{fig:Re-ordering} (b). 
If an instruction is identified as sensitive, the filtered results will be encapsulated and pushed into the FIFO queue. 
Otherwise, the instruction will be discarded, and an invalid packet (by setting the packet's lowest two bits to `0') will be generated and also pushed into the FIFO queues.
Also, we design the arbiter using a Finite State Machine (FSM) to transmit the buffered packets. 
The transmissions follow the method illustrated in Fig.~\ref{fig:Re-ordering} (c), consistently consuming one clock cycle for a valid packet while directly skipping the invalid packet.
Notably, buffering the invalid packets is required for maintaining synchronisation between the FIFO queues.

% s using the encapsulation format illustrated in Fig.\ref{fig:Encapsulation_Format}


\parlabel{Design trade-offs.}
Designing the event filter using the SRAM-based superscalar microarchitecture ensures that all instructions can be handled in the cycle following their commitment.
However, this approach necessitates deploying a mini-filter for each commit width of the main core, which may result in significant hardware overhead.

It is possible to shrink the usage of the mini-filters or even adopts a single-width filter~\cite{ainsworth2020guardian}.
To achieve this, the arbiter is required to be positioned between the main core and the filter(s) to schedule the filtering orders.
This approach decreases the parallelism levels of the filtering, may causing additional pipeline stalls of the main core. 
In \textcolor{blue}{Sec.~\ref{}}, we present a performance evaluation to examine the slowdown associated with event filters with different widths, assisting in the selection of the most suitable filtering configuration.




\subsection{Mapper}
\label{sbsc:Mapper}
The mapper creates high-efficiency communication channels throughout the system.
To this end, we develop the microarchitecture consisting of two primary components: a \emph{distributed} fabric network and an allocator. 
The fabric network provides dedicated data paths for transmitting filtered packets while also facilitating inter-checker communication. 
Concurrently, the allocator manages the scheduling and allocation of filtered packets from the event filter to the security checkers, leveraging the fabric network infrastructure for transmissions.
Below, we introduce their microarchitecture.

\parlabel{Microarchitecture}
Fig.~\ref{fig:Top_Micro} (d) illustrates the microarchitecture of the fabric network, which establishes a half-duplex multicast (1-to-N) channel and a full-duplex routing (N-to-N) channel.
The multicast channel \emph{selectively} broadcasts filtered packets to the security checkers, and the routing channel allows the checkers to communicate between each other.
We design the multicast channel using a set of multiplexers, directing the filtered packets from the event filter to the input data ports of these multiplexers, and connecting their output data ports to the message queues in the checkers. 
All the multiplexers are controlled by allocator, allowing the allocator to manage the transmission or masking of each filtered packet.
We design the routing channel using a Network-on-Chip (NoC) mesh, constructing the routers (\ie, transaction nodes) in a Manhattan grid, as described in~\cite{kumar2002network}. 
Each router features five 128-bit bi-directional ports, connected to other routers located to its north, south, east, and west, as well as to a security checker. 
The NoC mesh encapsulates on-chip transactions as packets using a protocol developed in~\cite{schoeberl2015t}, and employs wormhole-routing to direct the packets through each router towards their respective destinations.


Figure~\ref{fig:Mini_Filter} presents the microarchitecture of the allocator, comprising a distributor and a set of SEs.
The SEs are \emph{uniquely} linked to a guardian kernel, responsible for allocating packets to security checkers that are executing the same guardian kernel. 
The distributor manages the mapping between the SEs and the G$\_$IDs, deciding which SEs should be activated during packet transmission.
We design the distributor using bitmap registers and a multiplexer. 
A bitmap register is assigned to each G$\_$ID, and individual bits within the register are used to index the SEs that are interested in that specific G$\_$ID. 
For example, if SE$\_$0 needs to allocate packets with a particular G$\_$ID, the bit[0] of the corresponding G$\_$ID's bitmap should be set to `1'.
We connect the bitmap registers to input data ports of the multiplexer and direct the G$\_$ID returned by the event filter to the control port, allowing the selection of the appropriate bitmap when a packet is transmitted.
In coping with the broad types of guardian kernels, we design the SEs to support different scheduling policies.






\parlabel{Design trade-offs.}




\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{graphics/Allocator.pdf}
    \caption{Microarchitecture of allocator. As an example, 3 G\_IDs, 4 SEs are used to allocate filtered contents to 16 security checkers.}
    \label{fig:Mini_Filter}
\end{figure}


\subsection{Security checkers}
\label{sbsc:Security chckers}

\parlabel{ISAX interface.}

\parlabel{Hybrid duff's device.}

